A Performance-Driven Benchmark for Feature Selection in Tabular Deep Learning

Academic tabular benchmarks often contain small sets of curated features. In contrast, data scientists typically collect as many features as possible into their datasets, and even engineer new features from existing ones. To prevent overfitting in subsequent downstream modeling, practitioners commonly use automated feature selection methods that identify a reduced subset of informative features. Existing benchmarks for tabular feature selection consider classical downstream models, toy synthetic datasets, or do not evaluate feature selectors on the basis of downstream performance. Motivated by the increasing popularity of tabular deep learning, we construct a challenging feature selection benchmark evaluated on downstream neural networks including transformers, using real datasets and multiple methods for generating extraneous features. We also propose an input-gradient-based analogue of Lasso for neural networks that outperforms classical feature selection methods on challenging problems such as selecting from corrupted or second-order features.

==> tables/corrupted_table.tex <==
\begin{table}[t]
\caption{\textbf{Benchmarking feature selection methods for MLP and FT-Transformer downstream models on datasets with {\bf corrupted} extra features.} We report performance of models trained on features selected by different FS algorithms in terms of accuracy for classification and negative RMSE for regression problems. \% refers to percent of extra features in the dataset: either 50\% or 75\% features are corrupted. Bold font indicates the best numbers dataset-wise and lower rank indicates better overall performance.}
\label{tab:corrupted}
\centering
\scriptsize
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lllllllllllllll}
 \% & FS method + Model & AL & CH & CO & EY & GE & HE & HI & HO & JA & MI & OT & YE & rank \\
\midrule

50 & No FS + MLP & 0.946 & -0.475 & 0.965 & 0.557 & 0.525 & 0.370 & 0.802 & -0.607 & 0.703 & -0.909 & 0.778 & -0.797 & 5.58 \\

50 & Univariate + MLP & \textbf{0.955} & -0.451 & 0.966 & 0.556 & 0.514 & 0.346 & 0.810 & -0.620 & 0.717 & -0.920 & 0.795 & -0.828 & 5.08 \\

50 & Lasso + MLP & \textbf{0.955} & \textbf{-0.449} & 0.968 & 0.548 & 0.512 & 0.382 & 0.813 & -0.602 & 0.713 & -0.903 & 0.796 & -0.795 & 3.92 \\

50 & 1L Lasso + MLP & \textbf{0.955} & \textbf{-0.447} & 0.968 & 0.566 & 0.515 & 0.382 & 0.812 & -0.581 & 0.718 & -0.902 & 0.795 & -0.780 & 3.08 \\

50 & RF + MLP & 0.951 & -0.453 & 0.967 & 0.574 & \textbf{0.568} & 0.383 & 0.810 & -0.565 & \textbf{0.724} & -0.904 & 0.788 & -0.786 & 3.25 \\

50 & XGBoost + MLP & 0.954 & -0.454 & \textbf{0.969} & \textbf{0.583} & 0.510 & 0.384 & \textbf{0.815} & \textbf{-0.553} & 0.722 & \textbf{-0.892} & \textbf{0.803} & -0.779 & 2.08 \\

50 & Deep Lasso + MLP & \textbf{0.955} & \textbf{-0.447} & 0.968 & \textbf{0.577} & 0.525 & \textbf{0.388} & \textbf{0.815} & -0.567 & 0.721 & -0.895 & 0.801 & \textbf{-0.776} & {\bf 1.92} \\

\midrule
75 & No FS + MLP & 0.921 & -0.516 & 0.956 & 0.518 & 0.503 & 0.356 & 0.788 & -0.632 & 0.686 & -0.913 & 0.762 & -0.808 & 5.75 \\

75 & Univariate + MLP & 0.955 & -0.569 & 0.941 & 0.510 & 0.495 & 0.347 & 0.742 & -0.620 & 0.686 & -0.921 & 0.779 & -0.838 & 5.75 \\

75 & Lasso + MLP & 0.948 & -0.454 & 0.963 & \textbf{0.565} & 0.490 & 0.373 & 0.810 & -0.593 & 0.717 & -0.903 & 0.795 & -0.791 & 4.00 \\

75 & 1L Lasso + MLP & 0.955 & -0.444 & 0.967 & 0.549 & 0.495 & 0.380 & 0.811 & -0.576 & \textbf{0.715} & -0.903 & 0.797 & -0.779 & 2.58 \\

75 & RF + MLP & 0.952 & -0.450 & 0.963 & 0.547 & \textbf{0.533} & 0.372 & 0.805 & -0.573 & 0.716 & -0.903 & 0.765 & -0.788 & 3.83 \\

75 & XGBoost + MLP & 0.954 & -0.515 & \textbf{0.968} & \textbf{0.571} & \textbf{0.53} & 0.381 & 0.811 & \textbf{-0.571} & \textbf{0.721} & \textbf{-0.895} & 0.800 & -0.784 & 2.08 \\

75 & Deep Lasso + MLP & \textbf{0.959} & \textbf{-0.441} & \textbf{0.968} & 0.554 & 0.517 & \textbf{0.386} & \textbf{0.813} & \textbf{-0.563} & 0.718 & -0.898 & \textbf{0.804} & \textbf{-0.778} & {\bf 1.25} \\
\midrule 

50 & No FS + FT & 0.960 & -0.430 & 0.967 & 0.686 & 0.576 & 0.386 & 0.818 & -0.574 & 0.731 & -0.901 & 0.809 & -0.793 & 4.25\\

50 & Univariate + FT & \textbf{0.963} & \textbf{-0.422} & 0.965 & 0.681 & 0.574 & 0.345 & 0.812 & -0.628 & 0.733 & -0.920 & 0.812 & -0.826 & 4.33 \\

50 & Lasso + FT & 0.952 & \textbf{-0.422} & 0.936 & 0.697 & 0.556 & 0.387 & 0.820 & -0.586 & 0.732 & -0.937 & 0.812 & -0.915 & 4.50 \\

50 & AM + FT & 0.962 & -0.424 & 0.969 & 0.680 & 0.572 & \textbf{0.392} & 0.820 & \textbf{-0.549} & 0.734 & -0.901 & \textbf{0.817} & -0.790 & 2.56 \\

50 & RF + FT & 0.962 & \textbf{-0.422} & 0.969 & 0.711 & \textbf{0.6} & 0.387 & 0.819 & -0.557 & \textbf{0.735} & \textbf{-0.898} & 0.806 & -0.793 & 2.67 \\

50 & XGBoost + FT & \textbf{0.963} & \textbf{-0.422} & \textbf{0.97} & 0.706 & 0.564 & 0.392 & \textbf{0.821} & \textbf{-0.548} & \textbf{0.735} & \textbf{-0.897} & \textbf{0.816} & -0.790 & {\bf 1.83} \\

50 & Deep Lasso + FT & 0.961 & \textbf{-0.422} & 0.968 & \textbf{0.725} & 0.577 & \textbf{0.393} & \textbf{0.821} & -0.561 & \textbf{0.736} & \textbf{-0.898} & 0.809 & \textbf{-0.788} & 2.00 \\
\bottomrule

\end{tabular}
\end{table}

==> tables/random_table.tex <==
\begin{table}[t]

\caption{\textbf{Benchmarking feature selection methods for MLP and FT-Transformer downstream models on datasets with {\bf random} extra features.} We report performance of models trained on features selected by different FS algorithms in terms of accuracy for classification and negative RMSE for regression problems. \% refers to percent of extra features in the dataset: either 50\% or 75\% features are random. Bold font indicates the best numbers dataset-wise and lower rank indicates better overall result.}
\label{tab:random}
\centering
\scriptsize
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lllllllllllllll}
\toprule
 \%  & FS method & AL & CH & CO & EY & GE & HE & HI & HO & JA & MI & OT & YE & rank \\
\midrule
50 & No FS + MLP & 0.941 & -0.480 & 0.961 & 0.538 & 0.466 & 0.366 & 0.798 & -0.622 & 0.703 & -0.911 & 0.773 & -0.801 & 6.25 \\

50 & Univariate + MLP & \textbf{0.96} & -0.447 & \textbf{0.97} & 0.575 & 0.515 & 0.379 & 0.811 & \textbf{-0.549} & 0.715 & \textbf{-0.891} & \textbf{0.808} & -0.776 & {\bf 2.25} \\

50 & Lasso + MLP & 0.949 & -0.454 & \textbf{0.969} & 0.547 & 0.458 & 0.380 & 0.812 & -0.599 & 0.715 & -0.907 & 0.805 & -0.787 & 4.33 \\

50 & 1L Lasso + MLP & 0.952 & -0.451 & 0.969 & 0.564 & 0.474 & 0.375 & 0.811 & -0.568 & 0.715 & -0.897 & 0.796 & \textbf{-0.773} & 3.92 \\

50 & RF + MLP & 0.955 & -0.453 & 0.969 & \textbf{0.589} & \textbf{0.594} & \textbf{0.386} & \textbf{0.814} & -0.572 & \textbf{0.72} & -0.904 & 0.806 & -0.786 & 2.50 \\

50 & XGBoost + MLP & 0.956 & \textbf{-0.444} & 0.969 & \textbf{0.59} & 0.502 & \textbf{0.385} & 0.812 & -0.560 & \textbf{0.72} & -0.893 & 0.805 & -0.777 & 2.33 \\

50 & Deep Lasso + MLP & \textbf{0.959} & \textbf{-0.443} & 0.968 & 0.573 & 0.485 & 0.383 & 0.814 & \textbf{-0.549} & \textbf{0.72} & -0.894 & 0.802 & -0.776 & 2.50 \\
\midrule
75 & No FS + MLP & 0.925 & -0.527 & 0.955 & 0.502 & 0.417 & 0.348 & 0.778 & -0.674 & 0.671 & -0.917 & 0.749 & -0.812 & 6.17 \\

75 & Univariate + MLP & \textbf{0.96} & \textbf{-0.447} & \textbf{0.97} & 0.575 & 0.502 & 0.381 & 0.810 & \textbf{-0.549} & 0.713 & \textbf{-0.89} & \textbf{0.806} & -0.776 & 2.25 \\

75 & Lasso + MLP & 0.959 & -0.454 & 0.967 & 0.543 & 0.491 & 0.381 & 0.811 & -0.612 & 0.716 & -0.907 & 0.802 & -0.789 & 4.00 \\

75 & 1L Lasso + MLP & 0.957 & \textbf{-0.448} & 0.968 & 0.555 & 0.432 & 0.380 & 0.809 & -0.572 & 0.717 & -0.903 & 0.799 & \textbf{-0.775} & 4.00 \\

75 & RF + MLP & 0.949 & -0.453 & 0.968 & \textbf{0.584} & \textbf{0.61} & \textbf{0.386} & \textbf{0.814} & -0.585 & 0.718 & -0.902 & \textbf{0.808} & -0.784 & 2.50 \\

75 & XGBoost + MLP & 0.958 & -0.451 & \textbf{0.969} & 0.576 & 0.583 & 0.382 & 0.810 & -0.568 & \textbf{0.72} & -0.892 & 0.804 & \textbf{-0.774} & {\bf 1.92} \\

75 & Deep Lasso + MLP & 0.957 & \textbf{-0.446} & 0.969 & 0.569 & 0.479 & \textbf{0.387} & \textbf{0.814} & \textbf{-0.559} & \textbf{0.721} & -0.893 & 0.800 & \textbf{-0.774} & 2.33 \\

\midrule 


50 & No FS + FT & 0.959 & -0.432 & 0.966 & 0.673 & 0.500 & 0.384 & 0.817 & -0.577 & 0.730 & -0.902 & 0.813 & -0.792 & 5.00 \\

50 & Univariate + FT & \textbf{0.963} & -0.424 & \textbf{0.97} & 0.700 & 0.519 & 0.389 & 0.819 & \textbf{-0.554} & 0.733 & \textbf{-0.897} & 0.819 & -0.789 & 2.17 \\

50 & Lasso + FT & 0.952 & \textbf{-0.419} & 0.960 & 0.682 & 0.489 & 0.388 & 0.819 & -0.594 & 0.728 & -0.999 & 0.817 & -0.998 & 4.83 \\

50 & AM + FT & 0.962 & -0.425 & 0.968 & 0.657 & 0.505 & 0.389 & \textbf{0.82} & \textbf{-0.554} & 0.735 & -0.903 & 0.815 & \textbf{-0.789} & 3.08 \\

50 & RF + FT & 0.963 & \textbf{-0.42} & \textbf{0.969} & \textbf{0.718} & \textbf{0.591} & \textbf{0.395} & \textbf{0.821} & -0.558 & \textbf{0.737} & -0.900 & \textbf{0.82} & -0.791 & {\bf 1.58} \\

50 & XGBoost + FT & \textbf{0.963} & \textbf{-0.42} & \textbf{0.969} & \textbf{0.725} & 0.572 & 0.392 & \textbf{0.82} & -0.558 & 0.734 & \textbf{-0.898} & \textbf{0.82} & -0.789 & 1.67 \\



50 & Deep Lasso + FT & 0.962 & \textbf{-0.419} & \textbf{0.969} & 0.703 & 0.504 & 0.392 & \textbf{0.817} & -0.560 & 0.733 & -0.900 & 0.817 & \textbf{-0.788} & 2.67 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/random_table_recall.tex <==
\begin{table}[t]

\caption{\textbf{Recall scores for feature selection methods trained on datasets with random extraneous features} Bold font indicates the best numbers dataset-wise and lower rank indicates better overall result.}
\label{tab:random_recall}
\centering
\scriptsize
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lllllllllllllll}
\toprule
 \%  & FS method & AL & CH & CO & EY & GE & HE & HI & HO & JA & MI & OT & YE & rank \\
\midrule
50 & Univariate & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.808 & 0.844 & 0.963 & 0.786 & \textbf{1.0} & 0.648 & \textbf{0.986} & \textbf{1.0} & 0.967 & 2.75 \\

50 & Lasso & 0.987 & \textbf{1.0} & 0.989 & 0.704 & 0.403 & 0.963 & 0.750 & 0.875 & 0.661 & 0.588 & 0.969 & 0.922 & 5.00 \\

50 & 1L Lasso & 0.776 & \textbf{0.988} & 0.954 & 0.719 & 0.497 & 0.937 & 0.811 & 0.856 & 0.644 & 0.882 & 0.915 & 0.988 & 4.67 \\

50 & AGL & 0.946 & 0.738 & 0.794 & 0.777 & 0.469 & \textbf{0.989} & 0.704 & \textbf{1.0} & 0.665 & 0.870 & 0.875 & 0.987 & 4.50 \\

50 & LassoNet & \textbf{1.0} & \textbf{0.988} & \textbf{1.0} & 0.619 & 0.625 & \textbf{0.985} & 0.771 & 0.931 & 0.644 & 0.582 & 0.692 & 0.908 & 5.00 \\

50 & AM & 0.768 & \textbf{0.962} & 0.715 & 0.692 & 0.684 & \textbf{1.0} & 0.789 & 0.938 & 0.676 & 0.646 & 0.920 & 0.953 & 4.58 \\

50 & RF & 0.901 & \textbf{1.0} & 0.893 & 0.885 & \textbf{0.984} & \textbf{1.0} & 0.807 & 0.875 & 0.661 & 0.553 & 0.985 & 0.809 & 4.25 \\
50 & XGBoost & 0.945 & \textbf{1.0} & 0.944 & \textbf{0.969} & 0.894 & \textbf{1.0} & 0.818 & \textbf{1.0} & \textbf{0.981} & 0.956 & 0.992 & 0.977 & 2.17 \\

50 & Deep Lasso & \textbf{1.0} & \textbf{0.988} & 0.974 & 0.835 & 0.488 & \textbf{1.0} & \textbf{0.861} & \textbf{0.969} & 0.641 & 0.950 & \textbf{1.0} & \textbf{1.0} & 2.67 \\
\midrule 

75 & Univariate & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.769 & 0.688 & 0.963 & 0.643 & \textbf{1.0} & 0.537 & 0.987 & \textbf{1.0} & 0.967 & 2.67 \\

75 &Lasso & \textbf{1.0} & \textbf{1.0} & 0.957 & 0.608 & 0.766 & 0.963 & 0.679 & 0.812 & \textbf{0.622} & 0.401 & 0.963 & 0.878 & 3.75 \\

75 &1L Lasso & 0.882 & \textbf{0.975} & 0.909 & 0.665 & 0.231 & 0.948 & 0.632 & 0.881 & 0.531 & 0.721 & 0.933 & \textbf{0.996} & 5.17 \\

75 &AGL & 0.856 & \textbf{1.0} & 0.743 & 0.685 & 0.253 & 0.952 & 0.654 & 0.869 & 0.541 & 0.775 & 0.704 & 0.987 & 4.75 \\

75 &RF & 0.918 & \textbf{1.0} & 0.943 & \textbf{0.888} & \textbf{1.0} & \textbf{1.0} & \textbf{0.789} & 0.912 & 0.559 & 0.664 & 0.995 & 0.836 & 3.17 \\

75 &XGBoost & 0.938 & \textbf{1.0} & 0.946 & \textbf{0.873} & \textbf{0.994} & \textbf{1.0} & 0.643 & 0.938 & 0.567 & \textbf{0.993} & 0.974 & 0.981 & 2.67 \\

75 &Deep Lasso & 0.990 & \textbf{0.95} & 0.957 & 0.777 & 0.262 & \textbf{1.0} & \textbf{0.775} & 0.956 & 0.576 & 0.946 & 0.992 & \textbf{1.0} & 2.17\\

\bottomrule
\end{tabular}
\end{table}

==> tables/secondorder_table.tex <==
\begin{table}[t]
\caption{\textbf{Benchmarking feature selection methods for MLP and FT-Transformer downstream models on datasets with {\bf second-order} extra features.} We report performance of models trained on features selected by different FS algorithms in terms of accuracy for classification and negative RMSE for regression problems. \% refers to percent of extra features in the dataset: either 50\% or 75\% features are second-order. Bold font indicates the best numbers dataset-wise and lower rank indicates better overall result.}
\label{tab:secondorder}
\centering
\scriptsize
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lllllllllllllll}
 \% & FS method & AL & CH & CO & EY & GE & HE & HI & HO & JA & MI & OT & YE & rank \\
\midrule

50 & No FS + MLP & 0.960 & -0.443 & 0.969 & 0.631 & 0.605 & \textbf{0.383} & 0.811 & \textbf{-0.549} & 0.719 & -0.891 & 0.800 & -0.786 & 3.33 \\

50 & Univariate + MLP & \textbf{0.961} & -0.439 & 0.959 & 0.584 & 0.582 & 0.357 & 0.817 & -0.614 & 0.724 & -0.902 & 0.798 & -0.810 & 4.75 \\

50 & Lasso + MLP & 0.955 & -0.443 & 0.966 & 0.608 & 0.590 & 0.366 & 0.816 & -0.564 & 0.724 & -0.891 & \textbf{0.806} & -0.783 & 3.83 \\

50 & 1L Lasso + MLP & 0.959 & -0.445 & 0.969 & 0.634 & 0.571 & 0.380 & \textbf{0.815} & -0.565 & 0.728 & \textbf{-0.89} & \textbf{0.808} & -0.780 & 2.83 \\

50 & RF + MLP & 0.958 & \textbf{-0.437} & 0.969 & 0.639 & \textbf{0.619} & 0.370 & \textbf{0.818} & -0.586 & \textbf{0.735} & \textbf{-0.89} & 0.801 & -0.781 & 2.50 \\

50 & XGBoost + MLP & 0.870 & \textbf{-0.438} & \textbf{0.97} & 0.635 & 0.604 & 0.373 & \textbf{0.818} & -0.579 & \textbf{0.734} & \textbf{-0.891} & 0.805 & -0.786 & 2.75 \\

50 & Deep Lasso + MLP & \textbf{0.961} & \textbf{-0.441} & 0.969 & \textbf{0.648} & 0.600 & \textbf{0.384} & 0.815 & -0.572 & 0.733 & \textbf{-0.89} & \textbf{0.805} & \textbf{-0.776} &{\bf 2.17} \\

\midrule
75 & No FS + MLP & 0.952 & -0.451 & \textbf{0.969} & 0.630 & \textbf{0.598} & \textbf{0.388} & 0.808 & \textbf{-0.542} & 0.717 & -0.900 & 0.792 & -0.792 & 3.58 \\

75 & Univariate + MLP & 0.960 & -0.530 & 0.488 & 0.553 & 0.531 & 0.352 & 0.812 & -0.608 & 0.720 & -0.908 & 0.785 & -0.820 & 5.67 \\

75 & Lasso + MLP & \textbf{0.96} & \textbf{-0.434} & \textbf{0.968} & 0.612 & 0.519 & 0.363 & 0.820 & -0.554 & 0.739 & -0.894 & \textbf{0.807} & -0.793 & 3.08 \\

75 & 1L Lasso + MLP & \textbf{0.96} & -0.452 & 0.966 & \textbf{0.654} & 0.579 & 0.375 & 0.818 & -0.549 & \textbf{0.741} & -0.893 & 0.805 & -0.782 & 2.67 \\

75 & RF + MLP & 0.956 & -0.445 & 0.968 & 0.627 & 0.566 & 0.339 & 0.819 & -0.615 & 0.728 & -0.892 & 0.794 & -0.789 & 3.92 \\

75 & XGBoost + MLP & 0.459 & -0.495 & \textbf{0.968} & 0.627 & 0.555 & 0.358 & \textbf{0.821} & -0.588 & 0.738 & -0.892 & 0.803 & -0.795 & 4.00 \\

75 & Deep Lasso + MLP & 0.959 & -0.448 & \textbf{0.969} & \textbf{0.647} & 0.582 & 0.378 & \textbf{0.821} & -0.568 & \textbf{0.74} & \textbf{-0.89} & 0.805 & \textbf{-0.78} & {\bf 1.83} \\

\midrule
50 & No FS + FT & 0.962 & -0.425 & 0.968 & \textbf{0.733} & 0.558 & \textbf{0.391} & 0.819 & \textbf{-0.552} & 0.732 & -0.901 & \textbf{0.818} & -0.790 & 3.17\\

50 & Univariate + FT & \textbf{0.963} & \textbf{-0.419} & 0.942 & 0.615 & 0.573 & 0.351 & 0.820 & -0.613 & 0.728 & -0.910 & 0.810 & -0.819 & 4.83 \\

50 & Lasso + FT & 0.962 & -0.422 & 0.967 & 0.720 & 0.560 & 0.381 & \textbf{0.823} & -0.561 & 0.733 & -0.905 & 0.816 & -0.874 & 3.75 \\

50 & AM + FT & 0.963 & \textbf{-0.418} & \textbf{0.97} & 0.719 & 0.597 & 0.387 & 0.820 & -0.579 & 0.736 & -0.902 & \textbf{0.819} & -0.791 & 2.83 \\

50 & RF + FT & \textbf{0.963} & -0.422 & \textbf{0.97} & \textbf{0.733} & \textbf{0.615} & 0.365 & 0.822 & -0.600 & \textbf{0.738} & \textbf{-0.895} & 0.816 & -0.793 & 2.56 \\

50 & XGBoost + FT & 0.871 & -0.424 & 0.962 & \textbf{0.737} & 0.594 & 0.379 & 0.822 & -0.587 & 0.736 & \textbf{-0.896} & 0.812 & -0.792 & 3.42  \\


50 & Deep Lasso + FT & \textbf{0.963} & -0.422 & \textbf{0.97} & 0.726 & \textbf{0.608} & 0.388 & 0.822 & -0.558 & \textbf{0.738} & -0.897 & \textbf{0.819} & \textbf{-0.789} & {\bf 1.75}  \\

\bottomrule
\end{tabular}
\end{table}
